EdgeMatrix: A Resources Redefined Edge-Cloud System for Prioritized Services

The edge-cloud system has the potential to combine the advantages of heterogeneous devices and truly realize ubiquitous computing. However, for service providers to guarantee the Service-Level-Agreement (SLA) priorities, the complex networked environment brings inherent challenges such as multi-resource heterogeneity, resource competition, and networked system dynamics. In this paper, we design a framework for the edge-cloud system, namely EdgeMatrix, to maximize the throughput while guaranteeing various SLA priorities. First, EdgeMatrix introduces Networked Multi-agent Actor-Critic (NMAC) algorithm to redefine physical resources as logically isolated resource combinations, i.e., resource cells. Then, we use a clustering algorithm to group the cells with similar characteristics into various sets, i.e., resource channels, for different channels can offer different SLA guarantees. Besides, we design a multi-task mechanism to solve the problem of joint service orchestration and request dispatch (JSORD) among edge-cloud clusters, significantly reducing the runtime than traditional methods. To ensure stability, EdgeMatrix adopts a two-time-scale framework, i.e., coordinating resources and services at the large time scale and dispatching requests at the small time scale. The real trace-based experimental results verify that EdgeMatrix can improve system throughput in complex networked environments, reduce SLA violations, and significantly reduce the runtime than traditional methods.

==> TrainingAlgorithm.tex <==
\vspace{-0.3em}
\begin{algorithm}
	\caption{\small Training and Scheduling Process of \textit{KaiS}}
	\label{algorithm:global}
	\small Initialize the system environment and neural networks.
	
	
%	\For{\rm{slot} $t$ = $\left \langle0, 1, ...\right \rangle$}{
	\For{\rm{slot} $t$ = $1, 2, ...$}{

		
		\If {\rm{frame} $\tau$ \rm{begins}}{
			
			Get reward $\tilde{u}_{\tau-1}$ and store $[\tilde{\boldsymbol{s}}_{\tau-1}, \tilde{\boldsymbol{a}}_{\tau-1}, \tilde{u}_{\tau-1}] $;
			
			Use GNNs to embed system states as Eq. (\ref{equ:gnn embedding});
			
			%Select action $\tilde{\boldsymbol{a}}_{\tau}$ using $\pi_{\theta^{*}}(\cdot)$.
			Select $H$ high-value edge nodes $(\tilde{a}_{\tau}^{\bullet})$ and
			\linebreak compute their service scaling actions $(\tilde{\boldsymbol{a}}_{\tau}^{\star})$  \hspace*{3.0em}%
			\hbox{\raise 5pt \rlap{\smash{$\left.\begin{array}{@{  }c@{}}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\end{array}\color{orchestrator2}\right\}$}}}
			\hbox{\raise 9pt \rlap{\smash{$\color{orchestrator2}\begin{tabular}{l}\rotatebox{270}{\footnotesize \textbf{\textit{Orchestrate (GPG)}}}\end{tabular}$}}} 
			\linebreak using policy networks $\theta_g$ and $\theta_q$, respectively;
			
			
			Execute orchestration action $\tilde{\boldsymbol{a}}_{\tau} = (\tilde{a}_{\tau}^{\bullet}, \tilde{\boldsymbol{a}}_{\tau}^{\star})$;
			
			Update GNNs and policy networks using Eq. (\ref{equ:GNNDRL policy gradient});
		}
		
		 \ForPar{\rm{each eAP agent} $b \in B$ }{
			
			\If{ $\mathcal{Q}_{b} == \varnothing$}{
			
				\textbf{Continue}
			}
			
			Update request queue $\mathcal{Q}_{b}$ and get reward $\hat{u}_{b, t-1}$;
			
			Store $[ \hat{\boldsymbol{s}}_{b, t-1}, \hat{a}_{b, t-1}, A\left(\hat{\boldsymbol{s}}_{b, t-1}, \hat{a}_{b, t-1}\right),\hat{u}_{b, t-1},$
			\linebreak $ \boldsymbol{F}_{b, t-1}] $ for $\theta_{p}$ (actor);
			
			Dequeue current request $r_{b, t}$; 
			
			Compute the resource context $\boldsymbol{F}_{b, t}$ using Eq. (\ref{equ:resource context});\hspace*{1.0em}%
			\hbox{\raise -5pt \rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\end{array}\color{dispatchers2}\right\}$}}}
			\hbox{\raise -1pt \rlap{\smash{$\color{dispatchers2}\begin{tabular}{l}\rotatebox{270}{\textbf{\footnotesize \textit{Dispatch (cMMAC)}}}\end{tabular}$}}}
			
			Take dispatch action $\hat{a}_{b, t}$ for $r_{b,t}$ using Eq. (\ref{equ:probability of valid actions for agent});
			
		}
		
		Store $[ \hat{\boldsymbol{s}}_{t-1}, V^{*}\left(\hat{\boldsymbol{s}}_{t-1} ; \theta_{v}^{\prime}, \pi\right)] $ for $\theta_{v}$ (critic);
		
		Update neural networks $\theta_{p}$ (actor) and $\theta_{v}$ (critic) 
		\linebreak centrally using Eq. (\ref{equ:the gradient of policy of cMAAC}) and  (\ref{equ:loss function derived from Bellman equation}), respectively; 
		
		Synchronize $\theta_{p}$ periodically to distributed eAPs.
		
		
		
		
	} 
\end{algorithm}
\vspace{-0.6em}

